Reinforcing Chain-of-Thought Reasoning with Self-Evolving Rubrics

Despite chain-of-thought (CoT) playing crucial roles in LLM reasoning, directly rewarding it is difficult: training a reward model demands heavy human labeling efforts, and static RMs struggle with evolving CoT distributions and reward hacking. These challenges motivate us to seek an autonomous CoT rewarding approach that requires no human annotation efforts and can evolve gradually. Inspired by recent self-evolving training methods, we propose \textbf{RLCER} (\textbf{R}einforcement \textbf{L}earning with \textbf{C}oT Supervision via Self-\textbf{E}volving \textbf{R}ubrics), which enhances the outcome-centric RLVR by rewarding CoTs with self-proposed and self-evolving rubrics. We show that self-proposed and self-evolving rubrics provide reliable CoT supervision signals even without outcome rewards, enabling RLCER to outperform outcome-centric RLVR. Moreover, when used as in-prompt hints, these self-proposed rubrics further improve inference-time performance.

==> chapters/1_abstract.tex <==
\begin{abstract}
Chain-of-thought (CoT) plays a crucial role in LLM reasoning, yet outcome-centric reinforcement learning with verifiable rewards (RLVR) typically optimizes only final-answer correctness, leaving CoTs largely unrewarded and potentially inducing sub-optimal reasoning strategies. 
While important, directly rewarding CoT is challenging mainly for two practical reasons: training a reward model (RM) for CoT rewarding typically requires substantial human efforts, and a static RM may fail to align with the dynamic CoT distribution changes during training and also be vulnerable to reward hacking. 
These challenges motivate us to seek an autonomous CoT rewarding approach that requires no human annotation efforts and can evolve gradually. 
Inspired by recent self-evolving training methods, we propose \textbf{RLCER} (\textbf{R}einforcement \textbf{L}earning with \textbf{C}oT Supervision via Self-\textbf{E}volving \textbf{R}ubrics), which enhances the outcome-centric RLVR by rewarding CoTs with self-proposed and self-evolving rubrics.
We show that these self-proposed and self-evolving rubrics provide meaningful CoT supervision even without outcome rewards, and RLCER outperforms the vanilla outcome-centric RLVR across datasets and LLM backbones. 
Additionally, we demonstrate that the generated rubrics can also explicitly guide better reasoning, since using them as in-prompt hints further improves the LLM reasoning performance at inference time. 
\end{abstract}


